Efficient Structured Pruning and Architecture Searching for Group Convolution

Efficient inference of Convolutional Neural Networks is a thriving topic recently. It is desirable to achieve the maximal test accuracy under given inference budget constraints when deploying a pre-trained model. Network pruning is a commonly used technique while it may produce irregular sparse models that can hardly gain actual speed-up. Group convolution is a promising pruning target due to its regular structure; however, incorporating such structure into the pruning procedure is challenging. It is because structural constraints are hard to describe and can make pruning intractable to solve. The need for configuring group convolution architecture, i.e., the number of groups, that maximises test accuracy also increases difficulty. This paper presents an efficient method to address this challenge. We formulate group convolution pruning as finding the optimal channel permutation to impose structural constraints and solve it efficiently by heuristics. We also apply local search to exploring group configuration based on estimated pruning cost to maximise test accuracy. Compared to prior work, results show that our method produces competitive group convolution models for various tasks within a shorter pruning period and enables rapid group configuration exploration subject to inference budget constraints.

==> tex/method/heuristic.tex <==
\subsection{Heuristic Algorithm for Layer-wise Pruning}\label{sec:alg}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\columnwidth]{./figures/heuristic.pdf}
  \caption{
    Illustration of Algorithm~\ref{alg:greedy}.
    This algorithm runs at the 3rd diagonal block (in green), counting from the bottom-right one.
    Kernels covered by previous blocks (in red) are now frozen for further sorting (in gray).
    When updating the 3rd block, columns are sorted by sums-of-columns in range \textcircled{1} and then rows are sorted by sums-of-rows in range \textcircled{2}.}
  \label{fig:alg}
\end{figure}

%% Beginner
This section focuses on layer-wise pruning with given $G$.
We propose a heuristic algorithm, and it efficiently produce good enough solutions with regards to~\eqref{eq:opt}.
We justify the usability of this algorithm on randomly generated tests and statistics from real-world pre-trained CNN models.

\begin{algorithm}[!t]
  \caption{A greedy algorithm. The \texttt{sort} function sorts the given values in an increasing order, and returns permutation indices of the sorted array.}
  \label{alg:greedy}

  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
  \SetKwData{cols}{C}
  \SetKwData{rows}{R}
  \SetKwFunction{sort}{sort}

  \KwData{Weights $\W\in\mathbb{R}^{\CO\times\CI\times K_h\times K_w}$}
  \KwResult{$\IO$ and $\II$}

  $\II, \IO \gets \{1,\dots,\CI\}, \{1,\dots,\CO\}$\;
  \For{$f\in\{1,\dots, \CO \}$, $c\in\{1,\dots, \CI \}$}{
    $\widehat{\W}_{fc} \gets \norm{\W_{\IO(f)\II(c)}}$\;
  }

  % For each block
  \For{$g \gets \{G, \dots, 2, 1\}$}{\label{alg:greedy:block_loop}
    % TODO - change this i to a stabliser
    $\tilde{f} \gets \left\{
      \frac{(g-1)}{G}\CO + 1,\dots,\frac{g}{G}\CO\right\}$\;
    $\tilde{c} \gets \left\{
      \frac{(g-1)}{G}\CI + 1,\dots,\frac{g}{G}\CI\right\}$\;
    
    $\II^\prime \gets \sort(
      \left\{
        \sum\limits^{f\in\tilde{f}} \widehat{\W}_{\IO(f)\II(c)} \mid
        \forall c \leq \frac{g}{G}\CI
      \right\})$\;\label{alg:greedy:sort_in}
    \For{$c\gets \{1, \dots, \frac{g}{G}\CI\}$}{
      $\II(c)\gets \II(\II^\prime(c))$\;
    }
    
    $\IO^\prime \gets \sort(
      \left\{
        \sum\limits^{c\in\tilde{c}} \widehat{\W}_{\IO(f)\II(c)} \mid
        \forall f \leq \frac{g}{G}\CO
      \right\})$\;\label{alg:greedy:sort_out}
    \For{$f\gets \{1, \dots, \frac{g}{G}\CO\}$}{
      $\IO(f)\gets \IO(\IO^\prime(f))$\;
    }
  }
\end{algorithm}

\paragraph{Greedy algorithm by sorting.}
The objective in~\eqref{eq:opt} states that, we intend to permute the weights $\W$ by its input and output channels, so that the blocks remaining on the diagonal can retain most of the original importance.
Intuitively, this problem is difficult because a small change in permutation may affect values in several diagonal blocks.

We devise a greedy algorithm, listed as Algorithm~\ref{alg:greedy}, to address this challenge: we move the most important kernels towards one diagonal block at one time, and resolve others step by step (line~\ref{alg:greedy:block_loop}).
For each diagonal block, we \emph{sort} channels by their importance collected only from regions covered by the current block, denoted by $\tilde{f}$ and $\tilde{c}$, and those channels that may affect previously resolved blocks will be frozen (line~\ref{alg:greedy:sort_in} and \ref{alg:greedy:sort_out}).
\figref{fig:alg} illustrates this algorithm clearer.
Sorting once may not be sufficient, e.g., after we have sorted by output channels, kernels covered by input channels become different.
We empirically select a constant number $N_S$ that indicates the total rounds of sorting for each iteration, and we can place an inner loop under line~\ref{alg:greedy:block_loop}.
% Complexity analysis
The overall complexity of this algorithm is within polynomial time:
for each iteration, we need to do $N_S$ times of sorting and summing for input and output channels, and both sorting and summing use polynomial time.

%% NOTE: add this part when it is really effective
% \paragraph{Maximal bipartite matching.}


\begin{figure}[!t]
  \centering
  \includegraphics[width=\columnwidth]{figures/model_stats.pdf}
  \caption{Evaluation results on the heuristic algorithm. Recovery ratio is the percentage of magnitude, measured by L2 norm, retained in the diagonal blocks after pruning.}
  \label{fig:perf}
\end{figure}

\paragraph{Performance.}
We examine how this heuristic algorithm performs and results are summarised in \figref{fig:perf}.
The left includes results collected from 10,000 sample results. The input is a block-diagonal matrix randomly shuffled by channels, and we are expected to restore all entries back to the diagonal. As shown in~\figref{fig:perf}, most samples can be fully restored, especially when $N_S$ is 10.
We also run this algorithm on pre-trained ResNet-50\footnotemark{}:
as shown on the right, comparing with the baseline that does no sorting ($N_S$ is 0), our method can restore about 3\% more on all cases, which can improve the final test accuracy (Table~\ref{table:ablation:perm}).


% Older version
\begin{comment}
First, we check whether this algorithm can fully recover a randomly permuted matrix, the origin of which is a block diagonal matrix.
We have sampled 10,000 block diagonal matrices and randomly permuted them.
For each sample, we run our algorithm on it and collects the ratio of the sum of norms of remaining kernels over the sum of all norms.
We also explored whether $N_S$ will affect the performance.
All results are shown in \figref{fig:random:perf}: when $N_S$ is 10, around 70\% samples can be fully recovered; and most samples can be recovered by more than 90\%.

We then evaluate the actual performance on a real-world model, ResNet-50~\cite{He2015}, to see under different $G$ and $N_S$, how much magnitude can be retained by our algorithm.
In this case, we use a ResNet-50 model pre-trained on ImageNet\footnotemark.
\figref{fig:model:perf} illustrates the results: for each $G$ value, using our heuristic algorithm can achieve 2-3\% improvement in the ratio of retained magnitude.

This improvement looks trivial at this stage, mainly because the original pre-trained model has not been sparsified yet.
Therefore, removing such a large amount of kernels will normally reduce this much of magnitude.
% We have learned the permutations
However, it is worthwhile to note that we not only keep kernels with higher magnitude, but also learn the best pair of permutations.
Intuitively, retained kernels only contribute to the initialisation of the fine-tuning stage, but permutations have deeper effects on the network architectures.
%% TODO - elaborate this, we need to show how different permutation may affect the accuracy
Meanwhile, in later sections, we will show the significant improvement on the final model accuracy, which is a more decisive metric.
\end{comment}

\footnotetext{Pre-trained models are downloaded from \url{https://pytorch.org/docs/stable/torchvision/models.html}}


